Update on $B\to D^\ast \ell \nu$ form factor at zero-recoil using the Oktay-Kronfeld action

We present an update on the calculation of $\bar{B}\to D^\ast \ell \bar{\nu}$ semileptonic form factor at zero recoil using the Oktay-Kronfeld bottom and charm quarks on $N_f=2+1+1$ flavor HISQ ensembles generated by the MILC collaboration. Preliminary results are given for two ensembles with $a\approx 0.12$ and $0.09$ fm and $M_\pi\approx 310$ MeV. Calculations have been done with a number of valence quark masses, and the dependence of the form factor on them is investigated on the $a\approx 0.12$ fm ensemble. The excited state is controlled by using multistate fits to the three-point correlators measured at 4--6 source-sink separations.

==> tab_3pt/a09m310_m0074.tex <==
                 Unimp. & 4.64(12)     & 1.44  & 0.05  & 9.26(22)     & 0.90  & 0.63  & 5.49(10)     & 1.54  & 0.03  & 5.48(15)     & 0.68  & 0.91  \\ 
    $\CO(\lambda)$-imp. & 4.65(12)     & 1.44  & 0.05  & 9.27(22)     & 0.90  & 0.63  & 5.60(10)     & 1.54  & 0.03  & 5.60(15)     & 0.67  & 0.92  \\ 
  $\CO(\lambda^2)$-imp. & 4.42(12)     & 1.34  & 0.09  & 8.10(19)     & 0.84  & 0.73  & 5.33(10)     & 1.62  & 0.02  & 5.32(15)     & 0.76  & 0.83  \\ 


==> tab_3pt/a12m310_m0102.tex <==
                 Unimp. & 3.88(8)      & 1.20  & 0.21  & 8.44(17)     & 0.73  & 0.84  & 4.79(10)     & 0.73  & 0.84  & 4.84(11)     & 0.89  & 0.63  \\ 
    $\CO(\lambda)$-imp. & 3.89(8)      & 1.20  & 0.21  & 8.45(17)     & 0.73  & 0.84  & 4.90(10)     & 0.74  & 0.83  & 4.96(12)     & 0.84  & 0.70  \\ 
  $\CO(\lambda^2)$-imp. & 3.74(8)      & 1.27  & 0.15  & 7.50(15)     & 0.86  & 0.68  & 4.71(10)     & 0.73  & 0.84  & 4.79(11)     & 0.93  & 0.56  \\ 

